Contracting Skeletal Kinematics for Human-Related Video Anomaly Detection

Detecting the anomaly of human behavior is paramount to timely recognizing endangering situations, such as street fights or elderly falls. However, anomaly detection is complex since anomalous events are rare and because it is an open set recognition task, i.e., what is anomalous at inference has not been observed at training. We propose COSKAD, a novel model that encodes skeletal human motion by a graph convolutional network and learns to COntract SKeletal kinematic embeddings onto a latent hypersphere of minimum volume for Video Anomaly Detection. We propose three latent spaces: the commonly-adopted Euclidean and the novel spherical and hyperbolic. All variants outperform the state-of-the-art on the most recent UBnormal dataset, for which we contribute a human-related version with annotated skeletons. COSKAD sets a new state-of-the-art on the human-related versions of ShanghaiTech Campus and CUHK Avenue, with performance comparable to video-based methods. Source code and dataset will be released upon acceptance.

==> LaTeX/tables/experiment_table.tex <==
\begin{table}[!ht]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccc} 
\hline
\hline

& \multicolumn{1}{c}{\textbf{Video-based methods}}                                              &           \textbf{Params} &               \multicolumn{1}{c}{\textbf{UBnormal}}  &  \textbf{STC} &  \textbf{Avenue}  \\ 
\hline

\grayout{\textit{S}}& \grayout{\citen{Sultani} \cite{sultani18}} &   \grayout{-} & \grayout{50.3} &  \grayout{-} &  \grayout{-} \\ 
& \grayout{\citen{Georgescu}\cite{Georgescu21}}   & \grayout{$>80$M} &  \grayout{61.3} &  \grayout{-}  &  \grayout{-} \\ 
& \grayout{\citen{Bertasius}\cite{bertasius21}} & \grayout{121M} & \grayout{68.5} &  \grayout{-} &  \grayout{-} \\

\arrayrulecolor{gray}\hline\arrayrulecolor{black}\grayout{\textit{WS}} 

& \grayout{\citen{Georgescu} \cite{Georgescu21}} & \grayout{$>80$M}  & \grayout{59.3} & \grayout{82.7} & \grayout{92.3} \\

\arrayrulecolor{gray}\hline\arrayrulecolor{black}

\grayout{\textit{OCC}} & \grayout{\citen{Hasan} \cite{hasan16}}  &  \grayout{- }& \grayout{ - } & \grayout{70.4 } & \grayout{80.0 } \\
&  \grayout{\citen{Park} \cite{park2020learning}}  &  \grayout{-} & \grayout{-} & \grayout{69.8} & \grayout{82.8}       \\
&  \grayout{\citen{Liu} \cite{liu18}}  &  \grayout{14M} & \grayout{-} & \grayout{72.8} & \grayout{85.1}       \\
&  \grayout{\citen{Chang} \cite{chang2020clustering}}  &  \grayout{-} & \grayout{-} & \grayout{73.3} & \grayout{86.0}       \\
& \grayout{\citen{Barbalau} \cite{BARBALAU2023103656} } &  \grayout{$>80$M} &  \grayout{62.5}  & \grayout{83.8}  & \grayout{93.7}  \\

\hline
\hline

& \multicolumn{1}{c}{\textbf{Skeleton-based methods}} &  \textbf{Params} & \multicolumn{1}{c}{\textbf{HR-UBnormal}}  &  \textbf{HR-STC} &  \textbf{HR-Avenue} \\
\hline

\textit{OCC} & \citen{Morais} \cite{morais19} &  25K &  61.2  & 75.4 &  86.3 \\ 
& \citen{Markovitz} \cite{markovitz20} &  805K  &   55.2  & 74.8 &  58.1 \\
& \citen{Luo} \cite{luo19}  &  8M &  - & \underline{76.5} & \underline{87.3} \\
& Ours - \textit{radial} &  285K  & 63.4  & 75.2 &  82.2 \\
& Ours - \textit{Euclidean} & 240K &  \underline{65.2}  &  \textbf{\perfHRSTC} &  \textbf{87.8} \\
& Ours - \textit{hyperbolic}  & 240K & \textbf{65.5} &  75.6 & \underline{87.3} \\

\hline
\end{tabular}}
\caption{\added{Results on the human-related versions of the datasets UBnormal (\textit{HR-UBnormal}), ShanghaiTech Campus (\textit{HR-STC}) and CUHK Avenue (\textit{HR-Avenue)}, measured in terms of AUC score (bottom part of the table). We highlight in bold the best results and underline the second best. We report the results of video-based models on the non-HR versions of the aforementioned datasets (upper part of the table); it should be noted that such methods cannot be directly compared with skeleton-only ones, which are rather complementary, and hence are displayed in gray. The blocks split the table according to each method's framework, where \textit{S}, \textit{WS} and \textit{OCC} stand for \textit{Supervised}, \textit{Weakly-Supervised} and \textit{One Class Classification} methods, respectively.}}
\label{tab:stacked}

\end{table}

